On braided Hopf structures on exterior algebras

We show that the exterior algebra of a vector space $V$ of dimension greater than one admits a one-parameter family of braided Hopf algebra structures, arising from its identification with a Nichols algebra. We explicitly compute the structure constants with respect to a natural set-theoretic basis. A one-parameter family of diagonal automorphisms exists, which we use to construct solutions to the (constant) Yang--Baxter equation. These solutions are conjectured to give rise to the two-variable Links--Gould polynomial invariants associated with the super-quantum group $U_q(\mathfrak{gl}(N|1))$, where $N = \dim(V)$. We support this conjecture through computations for small values of $N$.

==> tikzext-util.tex <==
% Copyright 2024 by Qrrbrbirlbel
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%

\def\tikzextversion{0.6.2}
\def\tikzextversionnumber{10}
\def\tikzextset{\pgfqkeys{/tikz/ext}}
\def\pgfextset{\pgfqkeys{/pgf/ext}}
\pgfextset{
  pgf/.code=\pgfset{#1},
  .code=\pgfextset{#1}%
}
\tikzextset{
  tikz/.code=\tikzset{#1},
  .code=\tikzextset{#1},
  .unknown/.code={%
    \pgfextset{\pgfkeyscurrentname/.try={#1}}%
    \unless\ifpgfkeyssuccess
      \pgfutil@packageerror{tikz-ext}{%
        I neither know '/tikz/ext/\pgfkeyscurrentname' nor
        '/pgf/ext/\pgfkeyscurrentname' to which you passed '#1'.%
      }%
    \fi
  },
  /pgfplots/ext/.code=\tikzextset{#1},
  /pgfplots/ext/.unknown/.code={%
    \tikzextset{\pgfkeyscurrentname={#1}}%
  }
}
% Compatibility
\gdef\tikzextutil@compatwarning@counter{0}
\def\tikzextutil@compatmaybewarning#1#2#3{%
  \ifnum\tikzextutil@compatwarning@counter<25
    \xdef\tikzextutil@compatwarning@counter{\the\numexpr\tikzextutil@compatwarning@counter+1\relax}%
    \pgfutil@packagewarning{tikz-ext}{%
      The deprecated #1 was used. It is now #2. Please use that instead.^^J%
      To remove this warning use \string\tikzextset\string{compat/#3\string}.^^J%
      This warning will be removed in the next version and the #1 will fail.^^J%
    }%
  \else\ifnum\tikzextutil@compatwarning@counter=25
    \gdef\tikzextutil@compatwarning@counter{26}%
    \pgfutil@packagewarning{tikz-ext}{Too many warnings generated. Remain silent.}%
  \fi\fi
}
\def\tikzextutil@compatwarning@cmd#1#2#3#4#5{%
  \pgfutil@IfUndefined{#3}{%
    \pgfutil@namedef{#3}{%
      \tikzextutil@compatmaybewarning
        {command \expandafter\pgfutil@gobble\string\\#3}{\string#4}{#1 = #2}%
      #4%
    }%
  }{}%
}
\def\tikzextutil@compatwarning@key#1#2#3{%
  \pgfutil@ifnextchar[%
    {\tikzextutil@compatwarning@key@opt{#1}{#2}{#3}}%
    {\tikzextutil@compatwarning@key@   {#1}{#2}{#3}{}}%
}
\def\tikzextutil@compatwarning@key@opt#1#2#3[#4]{%
  \tikzextutil@compatwarning@key@{#1}{#2}{#3}{\pgfkeyssetvalue{#3/.@def}{#4}}%
}
\def\tikzextutil@compatwarning@key@#1#2#3#4#5{%
  \pgfkeys@pathtoks{#3}%
  \pgfkeysifdefined{#3}{%
    % The key is a value key. Do not overwrite or adjust.
    % Old TikZ-Ext key simply will not work.
  }{%
    \pgfkeysifdefined{#3/.@cmd}{%
      % The key is a code key. Do not overwrite or adjust.
      % Old TikZ-Ext key simply will not work.
    }{%
      % The key is currently not used.
      #4%
      \pgfkeysdef{#3}{%
        \tikzextutil@compatmaybewarning{key '#3'}{'#5'}{#1 = #2}%
        \pgfkeysvalueof{#5/.@cmd}##1\pgfeov
      }%
    }
  }
}
\def\tikzextutil@compatwarning@valuekey#1#2#3#4{%
  \pgfkeys@pathtoks{#3}%
  \pgfkeysifdefined{#3}{%
    % The key is a value key. Do not overwrite or adjust.
    % Old TikZ-Ext key simply will not work.
  }{%
    \pgfkeysifdefined{#3/.@cmd}{%
      % The key is a code key. Do not overwrite or adjust.
      % Old TikZ-Ext key simply will not work.
    }{%
      % The key is currently not used.
      \pgfkeyssetvalue{#3}{\pgfkeysvalueof{#4}}%
      \pgfkeysdef{#3}{%
        \tikzextutil@compatmaybewarning{value-key '#3'}{'#4'}{#1 = #2}%
        \pgfkeyssetvalue{#4}{##1}%
      }%
    }
  }
}
\def\tikzextutil@compatwarning@mathcmdZ#1#2#3#4{%
  \pgfutil@IfUndefined{pgfmath#3}{%
    \pgfmathdeclarefunction*{#3}{0}{%
      \tikzextutil@compatmaybewarning{PGFMath function '#3'}{'#4'}{#1 = #2}%
      \csname pgfmath#4@\endcsname
    }%
  }{}%
}
\def\tikzextutil@compatwarning@mathcmdI#1#2#3#4{%
  \pgfutil@IfUndefined{pgfmath#3}{%
    \pgfmathdeclarefunction*{#3}{1}{%
      \tikzextutil@compatmaybewarning{PGFMath function '#3'}{'#4'}{#1 = #2}%
      \csname pgfmath#4@\endcsname{##1}%
    }%
  }{}%
}
\def\tikzextutil@compatwarning@mathcmdII#1#2#3#4{%
  \pgfutil@IfUndefined{pgfmath#3}{%
    \pgfmathdeclarefunction*{#3}{2}{%
      \tikzextutil@compatmaybewarning{PGFMath function '#3'}{'#4'}{#1 = #2}%
      \csname pgfmath#4@\endcsname{##1}{##2}%
    }%
  }{}%
}
\def\tikzextutil@compatwarning@mathcmdX#1#2#3#4{%
  \pgfutil@IfUndefined{pgfmath#3}{%
    \pgfmathdeclarefunction*{#3}{...}{%
      \tikzextutil@compatmaybewarning{PGFMath function '#3'}{'#4'}{#1 = #2}%
      \csname pgfmath#4@\endcsname##1%
    }%
  }{}%
}
\def\tikzextutil@compatwarning@handler#1#2#3#4{%
  \pgfkeys@pathtoks{/handlers/#3}%
  \pgfkeysifdefined{/handlers/#3}{%
    % The key is a value key. Do not overwrite or adjust.
    % Old TikZ-Ext key simply will not work.
  }{%
    \pgfkeysifdefined{/handlers/#3/.@cmd}{%
      % The key is a code key. Do not overwrite or adjust.
      % Old TikZ-Ext key simply will not work.
    }{%
      % The key is currently not used.
      \pgfkeysdef{/handlers/#3}{%
        \tikzextutil@compatmaybewarning{handler '#3'}{'#4'}{#1 = #2}%
        \pgfkeysvalueof{/handlers/#4/.@cmd}##1\pgfeov
      }%
    }
  }
}
\def\tikzextutil@compat@cloneshape#1#2{%
  \pgfutil@namelet{pgf@sh@s@#1}{pgf@sh@s@ext_#1}%
  \def\tikzext@temp{\edef\pgf@sm@shape@name{ext_#1}}%
  \expandafter\tikzextutil@prefix@macrotomacro\csname pgf@sh@s@#1\endcsname\tikzext@temp
  \pgfutil@namelet{pgf@anchor@#1@border}{pgf@anchor@ext_#1@border}%
  \pgfutil@namelet{pgf@sh@boxes@#1}{pgf@sh@boxes@ext_#1}%
  \pgfutil@for\tikzext@temp:=#2\do{%
    \pgfutil@namelet{pgf@anchor@#1@\tikzext@temp}{pgf@anchor@ext_#1@\tikzext@temp}}%
  \pgfutil@for\tikzext@temp:=bbg,bg,fbg,fg,ffg\do{%
    \pgfutil@namelet{pgf@sh@\tikzext@temp @#1}{pgf@sh@\tikzext@temp @ext_#1}}}

\tikzextset{
  compat/.is choice, compat/.default=warn,
  /tikz-ext/compat/add library/.code 2 args={%
    \tikzextset{
      compat/#1/.is choice,
      compat/#1/.default=#2,
      compat/#1/0.6.1/.style={/tikz/ext/compat/#1/0.6},
      compat/#1/0.6.2/.style={/tikz/ext/compat/#1/0.6}}%
    \pgfutil@for\tikzext@temp:=pre 0.6,0.6,0.6.1,0.6.2,newest,warn\do{%
      \pgfkeys@expanded{%
        \noexpand\tikzextset{%
          compat/\tikzext@temp/.append style=%
            /tikz/ext/compat/#1/\tikzext@temp}}%
      \pgfkeysedef
        {/tikz/ext/compat/#1/\tikzext@temp}
        {\noexpand\pgfkeyssetvalue{/tikz/ext/compat/#1}{\tikzext@temp}}%
    }%
  },
}

\def\tikzext@temp#1{%
  \pgfkeysedef{/tikz/ext/compat/#1}{%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/arrows}                {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/pgffor}                {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/misc}                  {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/nodes}                 {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/node-families}         {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/patterns.images}       {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/paths.arcto}           {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/paths.ortho}           {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/paths.timer}           {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/pgffor-ext}            {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/pgfkeys-plus}          {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/positioning-plus}      {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/pgfcalendar-ext}       {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/scalepicture}          {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/shapes}                {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/topaths.arcthrough}    {#1}%
    \noexpand\pgfkeyssetvalue{/tikz/ext/compat/transformations.mirror}{#1}%
  }}
\tikzext@temp{pre 0.6}
\tikzext@temp{0.6}
\tikzextset{
  compat/0.6.1/.style={/tikz/ext/compat/0.6},
  compat/0.6.2/.style={/tikz/ext/compat/0.6}%
}
\tikzext@temp{newest}
\tikzext@temp{warn}
\tikzextset{compat=warn}

\long\def\tikzextutil@gobblethree#1#2#3{}
\def\tikzextutil@addto@macro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}} % calendar: if
\def\tikzextutil@prefixtomacro#1#2{%
  \def\tikzext@temp{#2}%
  \tikzextutil@prefix@macrotomacro#1\tikzext@temp
}
\def\tikzextutil@prefix@macrotomacro#1#2{%
  \expandafter\expandafter\expandafter\def
  \expandafter\expandafter\expandafter#1%
  \expandafter\expandafter\expandafter{\expandafter#2#1}}

\def\tikzextutil@firstofmany#1#2\pgf@stop{#1}
\def\tikzextutil@secondofmany#1#2\pgf@stop{#2}
\endinput


==> tikzlibraryext.arrows-plus.code.tex <==
% Copyright 2024 by Qrrbrbirlbel
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%

\unless\ifcsname tikzextset\endcsname
  \input tikzext-util.tex
\fi


% \tikzext@arrow@evalshift
%
% Stores the shift amount into \tikzext@arrow@shift@
%
\def\tikzext@arrow@evalshift#1#2#3{%
  \pgf@arrow@compute@shortening#1%
  \ifcase\pgfkeysvalueof{/tikz/ext/arrow/shift mode}\relax
    \def#3{0pt}%
  \or
    \pgfmathsetlengthmacro#3%
      {(\pgfkeysvalueof{/tikz/ext/arrow shift factor #2})*-\pgf@xb}%
  \or
    \pgfmathsetlengthmacro#3%
      {(\pgfkeysvalueof{/tikz/ext/arrow shift factor #2})*-\pgf@xa}%
  \fi
}


% For bended arrows the shifting can't simply be done by a transformation
\def\tikzext@arrow@sneak#1\pgf@stop#2#3{% TODO
  \unless\ifdim#3=0pt
    \def#2{#1\pgf@arrow@handle{_}{\pgfarrowsep=#3\relax}}%
  \fi
}

%
% Arrow keys
%
\pgfkeysdef{/tikz/ext/pos > angle}{%
  \pgfkeysvalueof{/tikz/pos/.@cmd}(#1-\tikz@timer@start@angle)/(\tikz@timer@end@angle-\tikz@timer@start@angle)\pgfeov}
\tikzextset{%
  every softpath arrows/.code=
    \pgfkeysdef{/tikz/pos >}{\pgfkeysvalueof{/tikz/pos/.@cmd}##1\pgfeov}%
    \pgfkeysdef{/tikz/pos <}{\pgfkeyssetvalue{/tikz/ext/pos <}{##1}},
  every arc arrows/.code=
    \pgfkeysdef{/tikz/pos > angle}{\pgfkeysvalueof{/tikz/ext/pos > angle/.@cmd}##1\pgfeov}%
    \pgfkeysdef{/tikz/pos < angle}{\pgfkeysvalueof{/tikz/ext/pos < angle/.@cmd}##1\pgfeov}%
    \pgfkeysdef{/tikz/pos >}{\pgfkeysvalueof{/tikz/pos/.@cmd}##1\pgfeov}%
    \pgfkeysdef{/tikz/pos <}{\pgfkeyssetvalue{/tikz/ext/pos <}{##1}},
  pos < angle/.code=\pgfkeyssetvalue{/tikz/ext/pos <}{(#1-\tikz@timer@start@angle)/(\tikz@timer@end@angle-\tikz@timer@start@angle)},
  softpath arrows/.default=,
  softpath arrows/.code={%
    \begingroup
      \tikzset{ext/every softpath arrows,#1}%
      \pgfsyssoftpath@getcurrentpath\tikz@temp
      \pgfprocesssplitsubpath\tikz@temp
      \expandafter\pgf@parse@end\pgfprocessresultsubpathsuffix\pgf@stop\pgf@stop\pgf@stop
      \tikzext@arrow@softpath@curve
      \setbox\tikz@whichbox=\hbox\bgroup
        \unhbox\tikz@whichbox
        \hbox\bgroup\bgroup
          \pgfinterruptpath
          \pgfscope
            \pgfutil@ifxempty\pgf@start@tip@sequence{}{%
              \tikzext@arrow@evalshift\pgf@start@tip@sequence{start}\tikzext@arrow@shift@start
              \expandafter\tikzext@arrow@sneak\pgf@start@tip@sequence\pgf@stop\pgf@start@tip@sequence\tikzext@arrow@shift@start
            }%
            \pgfutil@ifxempty\pgf@end@tip@sequence{}{%
              \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
              \expandafter\tikzext@arrow@sneak\pgf@end@tip@sequence\pgf@stop\pgf@end@tip@sequence\tikzext@arrow@shift@end
            }%
            \pgfset{tips}%
            \pgftransformreset
            \tikzext@arrow@softpath
            \pgfusepath{}%
          \endpgfscope
          \endpgfinterruptpath
        \egroup\egroup
      \egroup
    \global\setbox\tikz@tempbox=\box\tikz@whichbox%
    \expandafter\endgroup%
    \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox%
  },
  arc arrows/.default=,
  arc arrows/.code={%
    \ifx\tikz@timer\tikz@timer@arc
      \begingroup
        \tikzset{ext/every arc arrows,#1}%
        \setbox\tikz@whichbox=\hbox\bgroup
          \unhbox\tikz@whichbox
          \hbox\bgroup\bgroup
            \pgfinterruptpath
            \pgfscope
              \pgfutil@ifxempty\pgf@start@tip@sequence{}{%
                \tikzext@arrow@evalshift\pgf@start@tip@sequence{start}\tikzext@arrow@shift@start
                \expandafter\tikzext@arrow@sneak\pgf@start@tip@sequence\pgf@stop\pgf@start@tip@sequence\tikzext@arrow@shift@start
              }%
              \pgfutil@ifxempty\pgf@end@tip@sequence{}{%
                \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
                \expandafter\tikzext@arrow@sneak\pgf@end@tip@sequence\pgf@stop\pgf@end@tip@sequence\tikzext@arrow@shift@end
              }%
              \pgfset{tips}%
              \tikzext@arrow@arcpath
              \pgfusepath{}%
            \endpgfscope
            \endpgfinterruptpath
          \egroup\egroup
        \egroup
      \global\setbox\tikz@tempbox=\box\tikz@whichbox
      \expandafter\endgroup
      \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox
    \else
      \pgfutil@packagewarning{tikz-ext}
        {arc arrow used on non-arc path segment, using ``softpath arrows'' instead}%
      \tikzset{ext/softpath arrows={#1}}%
    \fi
  },
  pos </.initial=0.0,
  pos >/.style={/tikz/pos={#1}},
  arrow shift mode/.is choice,
  arrow shift mode/off/.code                  =\pgfkeyssetvalue{/tikz/ext/arrow/shift mode}{0},
  arrow shift mode/total length/.code         =\pgfkeyssetvalue{/tikz/ext/arrow/shift mode}{1},
  arrow shift mode/total/.code                =\pgfkeyssetvalue{/tikz/ext/arrow/shift mode}{1},
  arrow shift mode/length until line end/.code=\pgfkeyssetvalue{/tikz/ext/arrow/shift mode}{2},
  arrow shift mode/line end/.code             =\pgfkeyssetvalue{/tikz/ext/arrow/shift mode}{2},
  arrow shift mode=total length,
  arrow shift factor/.code=\pgfkeyssetvalue{/tikz/ext/arrow shift factor start}{#1}%
                           \pgfkeyssetvalue{/tikz/ext/arrow shift factor end}{#1},
  arrow shift factor start/.initial=.5,
  arrow shift factor end/.initial=.5
}
%
% Arrow pics
%
\tikzset{
  pics/ext/arrow/.default=,
  pics/ext/arrow/.style={
    /tikz/sloped, /tikz/allow upside down,
    foreground code=, background code=, setup code=,
    code=%
      \edef\tikzext@temp{#1}%
      \pgfutil@ifxempty\tikzext@temp{}{%
        \pgfsetarrowsend{#1}%
      }%
      \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
      \pgftransformxshift{+-\tikzext@arrow@shift@end}%
      \pgf@arrow@draw@arrow\pgf@end@tip@sequence\pgf@xb
  },
  pics/ext/softpath arrow/.default=,
  pics/ext/softpath arrow/.code={%
    \let\pgf@start@tip@sequence\pgfutil@empty
    \edef\tikzext@temp{#1}%
    \pgfutil@ifxempty\tikzext@temp{}{%
      \pgfsetarrowsend{#1}%
    }%
    \pgfqkeys{/tikz/pics}{ext/softpath arrows}%
  },
  pics/ext/softpath arrows/.default=,
  pics/ext/softpath arrows/.style={
    foreground code=, background code=,
    setup code={%
      \edef\tikzext@temp{#1}%
      \pgfutil@ifxempty\tikzext@temp{}{%
        \pgfsetarrows{#1}%
      }%
      \pgfutil@ifxempty\pgf@start@tip@sequence{}{%
        \tikzext@arrow@evalshift\pgf@start@tip@sequence{start}\tikzext@arrow@shift@start
        \expandafter\tikzext@arrow@sneak\pgf@start@tip@sequence\pgf@stop\pgf@start@tip@sequence\tikzext@arrow@shift@start
      }%
      \pgfutil@ifxempty\pgf@end@tip@sequence{}{%
        \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
        \expandafter\tikzext@arrow@sneak\pgf@end@tip@sequence\pgf@stop\pgf@end@tip@sequence\tikzext@arrow@shift@end
      }%
      \pgfsyssoftpath@getcurrentpath\tikz@temp
      \pgfprocesssplitsubpath\tikz@temp
      \expandafter\pgf@parse@end\pgfprocessresultsubpathsuffix\pgf@stop\pgf@stop\pgf@stop
      \tikzext@arrow@softpath@curve
    },
    code=%
      \pgfset{tips}%
      \pgftransformreset
      \tikzext@arrow@softpath
      \pgfusepath{}%
  }
}

% curve
\def\tikzext@arrow@softpath@curve{%
  \ifx\pgfpointthirdlastonpath\relax
    \let\tikzext@arrow@softpath\tikzext@arrow@linepath
  \else
    \let\tikzext@arrow@softpath\tikzext@arrow@curvepath
  \fi
}
%
% Paths
%
% Line
\def\tikzext@arrow@linepath{%
  \pgfpathmoveto{%
    \pgfpointlineattime
      {\pgfkeysvalueof{/tikz/ext/pos <}}
      {\pgfpointsecondlastonpath}
      {\pgfpointlastonpath}%
  }%
  \pgfpathlineto{%
    \pgfpointlineattime
      {\tikz@time}
      {\pgfpointsecondlastonpath}
      {\pgfpointlastonpath}%
  }%
}
% Curve
\def\tikzext@arrow@curvepath{%
  \pgfpathcurvebetweentime
    {\pgfkeysvalueof{/tikz/ext/pos <}}
    {\tikz@time}
    {\pgfpointfourthlastonpath}
    {\pgfpointthirdlastonpath}
    {\pgfpointsecondlastonpath}
    {\pgfpointlastonpath}%
}

\def\tikzext@arrow@arcpath{%
  \pgfmathcos@{\tikz@timer@start@angle}%
  \let\tikz@angle@cos\pgfmathresult
  \pgfmathsin@{\tikz@timer@start@angle}%
  \let\tikz@angle@sin\pgfmathresult
  \pgfpathmoveto{%
    \pgfpointarcaxesattime
      {\pgfkeysvalueof{/tikz/ext/pos <}}
      {\pgfpointdiff{%
          \pgfpointadd{\pgfpointscale{\tikz@angle@cos}{\tikz@timer@zero@axis}}
                      {\pgfpointscale{\tikz@angle@sin}{\tikz@timer@ninety@axis}}}{\tikz@timer@start}}
      {\tikz@timer@zero@axis}
      {\tikz@timer@ninety@axis}
      {\tikz@timer@start@angle}
      {\tikz@timer@end@angle}%
  }%
  \pgfpatharcaxes
    {(\tikz@timer@end@angle-\tikz@timer@start@angle)*%
      (\pgfkeysvalueof{/tikz/ext/pos <})+\tikz@timer@start@angle}
    {(\tikz@timer@end@angle-\tikz@timer@start@angle)*%
      (\tikz@time)+\tikz@timer@start@angle}
    {\tikz@timer@zero@axis}
    {\tikz@timer@ninety@axis}%
}
%
% \arrow(reversed)*(*) macro for decoration.markings
%
\def\pgf@lib@dec@doarrowhead{%
  \pgfutil@ifnextchar*%
    {\tikzext@lib@dec@doarrowhead{1}}
    {\pgfutil@ifnextchar[%
      {\tikz@lib@dec@doarrowhead}
      {\tikz@lib@dec@doarrowhead[]}%
    }%
}
\def\pgf@lib@dec@doarrowheadrev{%
  \pgfutil@ifnextchar*%
    {\tikzext@lib@dec@doarrowhead{-1}}
    {\pgfutil@ifnextchar[%
      {\tikz@lib@dec@doarrowheadrev}
      {\tikz@lib@dec@doarrowheadrev[]}%
    }%
}

\def\tikzext@lib@dec@doarrowhead#1*{%
  \pgfutil@ifnextchar*%
    {\tikzext@lib@dec@doarrowhead@@{#1}}
    {\pgfutil@ifnextchar[%
      {\tikzext@lib@dec@doarrowhead@{#1}}
      {\tikzext@lib@dec@doarrowhead@{#1}[]}}%
}
\def\tikzext@lib@dec@doarrowhead@#1[#2]#3{%
  \scope[{#2}]%
    \pgfsetarrowsend{#3}%
    \pgfutil@ifxempty\pgf@end@tip@sequence{}{%
      \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
      \pgftransformxscale{#1}%
      \pgftransformxshift{+-\tikzext@arrow@shift@end}%
      \pgf@arrow@draw@arrow\pgf@end@tip@sequence\pgf@xb
    }%
  \endscope
}
\def\tikzext@lib@dec@doarrowhead@@#1*{%
  \pgfutil@ifnextchar[%]
    {\tikzext@lib@dec@doarrowhead@@@{#1}}
    {\tikzext@lib@dec@doarrowhead@@@{#1}[]}%
}

\def\tikzext@lib@dec@doarrowhead@@@#1[#2]#3{%
  \ifx\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentcurveto
    \pgftransformreset
    \pgfset{tips}%
    \ifnum#1<0
      \pgfsetarrows{[reversed]}%
    \fi
    \scope[{#2}]%
      \pgfsetarrowsend{#3}%
      \pgfutil@ifxempty\pgf@end@tip@sequence{}{%
        \tikzext@arrow@evalshift\pgf@end@tip@sequence{end}\tikzext@arrow@shift@end
        \expandafter\tikzext@arrow@sneak\pgf@end@tip@sequence\pgf@stop\pgf@end@tip@sequence\tikzext@arrow@shift@end
        \ifdim\pgf@decorate@inputsegmenttime pt=1pt % something weird for 1.0
          \def\pgf@decorate@inputsegmenttime{1}%
        \fi
        \ifdim\pgf@decorate@inputsegmenttime pt<0.05pt % zero is bad
          \def\pgf@decorate@inputsegmenttime{0.05}%
        \fi
        \pgfpathcurvebetweentime{0}{\pgf@decorate@inputsegmenttime}%
            {\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
            {\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
        \pgfusepath{}%
      }%
    \endscope
  \else
    \tikzext@lib@dec@doarrowhead@{#1}[{#2}]{#3}%
  \fi
}
\endinput
